ASCENT-ViT: Attention-based Scale-aware Concept Learning Framework for Enhanced Alignment in Vision Transformers

As Vision Transformers (ViTs) are increasingly adopted in sensitive vision applications, there is a growing demand for improved interpretability. This has led to efforts to forward-align these models with carefully annotated abstract, human-understandable semantic entities - concepts. Concepts provide global rationales to the model predictions and can be quickly understood/intervened on by domain experts. Most current research focuses on designing model-agnostic, plug-and-play generic concept-based explainability modules that do not incorporate the inner workings of foundation models (e.g., inductive biases, scale invariance, etc.) during training. To alleviate this issue for ViTs, in this paper, we propose ASCENT-ViT, an attention-based, concept learning framework that effectively composes scale and position-aware representations from multiscale feature pyramids and ViT patch representations, respectively. Further, these representations are aligned with concept annotations through attention matrices - which incorporate spatial and global (semantic) concepts. ASCENT-ViT can be utilized as a classification head on top of standard ViT backbones for improved predictive performance and accurate and robust concept explanations as demonstrated on five datasets, including three widely used benchmarks (CUB, Pascal APY, Concept-MNIST) and 2 real-world datasets (AWA2, KITS).

==> content/introduction_alignment.tex <==
\section{Introduction}
\label{sec:intro}

% Notes on alignment
With the surge of advanced deep learning methods, Deep Neural Networks (DNNs), especially Transformer-based models \cite{vaswani2017attention}, have been widely deployed to improve multiple facets of human endeavors \cite{dargan2020survey,shorten2021deep}. With the recent advancements in efficient training of transformer-based architectures \cite{devlin2018bert}, such large-scale models have revolutionized Computer Vision Applications \cite{dosovitskiy2020image}, time-series analysis \cite{gu2023mamba}, etc. Research in developing high-performing, generalizable, and efficient architectures has led to experts classifying a family of fundamental architectures as `Foundation Models' \cite{bommasani2021opportunities}. These foundation models are generally pre-trained on enormous amounts of unstructured data using weakly- or self-supervised learning paradigms that enable efficient data ingestion and processing which eases the process of learning relationships from data representations. In computer vision, Vision Transformers (ViT) \cite{dosovitskiy2020image} show great scalability and impressive performance in various downstream tasks, which promotes its use in real-world applications like autonomous driving \cite{ando2023rangevit,dong2021image}.


Ever since the advent of the first Artificial Intelligence (AI) systems, ensuring \textbf{AI alignment} \cite{gabriel2020artificial} has been a long-standing ideal to achieve. Although AI alignment is a broad term, most experts define it as ``designing AI systems which behave in line with human intentions and values'' \cite{ji2023ai}. In other words, AI systems should attempt to closely incorporate human thought and reasoning into their decision-making process. However, with ever-increasing foundation model sizes and no direct human supervision during pre-training, several experts have expressed grave concerns about the risk of \textbf{misalignment} of such models. One such popular example is detailed in \citet{hendricks2018women}, where models unknowingly amplify biases in the training data. To effectively reduce misalignment, the focus has been on both evaluating the extent of misalignment by posthoc interpretability approaches (\textbf{backward alignment}) or designing systems that intrinsically incorporate human-in-the-loop reasoning (\textbf{forward alignment}). The problem of alignment is much more pronounced in present-day large-scale DNNs like ViTs. As pre-training of ViTs is done on unstructured data, it is very hard to control misalignment, a problem pointed out in \citet{caron2021emerging}.

Forward Alignment includes a class of methods that try to design intrinsically interpretable models. One possible method to achieve alignment for vision models is utilizing human-annotated `concepts' to align model representations. Concepts can be considered as shared abstract entities across multiple instances, which provide a general understanding of the task processed by the model. Concepts are fundamental to human vision perception, wherein humans can effortlessly make semantic similarities between different objects by linking them through shared concepts. As a result, concept-based explainability has been successful in explaining DNN predictions \cite{koh2020concept,kim2018interpretability,li2018deep,alvarez2018towards,chen2019looks} and has been used to design intrinsically explainable models. As a result, many studies have attempted to \textit{align} model representations with concept annotations using concept-based explainability modules.


The problem of designing a system to align concepts with model representations can be formulated as a 2-step process. Given a set of concept representations $C$ associated with an input sample $x$, the task prediction is dependent on $y = g(C)$ where $g$ is any interpretable function used to aggregate concepts. To ensure maximum alignment, the set $C$ is annotated with human annotations and is used to supervise the training procedure. Multiple works such as \citet{alvarez2018towards} and \citet{agarwal2021neural} have postulated using a weighted linear sum of concepts as $g$ or utilizing a shallow feed-forward network \cite{koh2020concept}. With the success of attention mechanism \cite{vaswani2017attention}, approaches like \citet{wang2023learning, rigotti2021attention} directly supervise an attention matrix with annotated concept maps.


Concept-based explainability approaches are usually designed to be model-agnostic \cite{koh2020concept} and plug-and-play \cite{rigotti2021attention} to fit all possible use cases. However, this approach is fundamentally flawed as not all model representations can be treated similarly. For example, even though ViTs demonstrate impressive results, they are demonstrated to be scale-sensitive \cite{xu2021vitae}, a known strength of classical vision architectures like CNNs. Researchers have attempted to improve ViTs by incorporating CNN-like inductive biases in their architectures with great success \cite{liu2021swin,graham2021levit}. However, the majority of explainability research do not offer a nuanced analysis by incorporating such model-specific inductive biases in the explainability modules. As discussed in \citet{xu2021vitae}, the role of image scale is important in learning more robust representations. As a consequence, we augment present attention-based explainability modules with multi-scale features to improve the alignment of model representations with concepts. Our proposed approach is therefore an attempt to combine inductive biases from CNNs and ViTs in a concept-based explainability module.


In this paper, we propose \textbf{Attention-based Concept Alignment Module (ACAM)}, a concept-based explainability module for ViTs to \textit{align} human-annotated concepts with model representations. Unlike model-agnostic plug-and-play explainability modules which, by definition do not respect inductive biases of the models, ACAM effectively composes inductive biases of CNNs and ViTs - scale invariance and image-patch relationship awareness respectively into learned representations. More precisely, ACAM consists of 3 distinct modules - (i) Scale Awareness Module which models concepts at various scales, (ii) Multi-scale Feature Interaction Module which composes multi-scale concepts with patch embeddings, and (iii) Concept Attention Module which aligns concepts with the learned model representations. To summarize, our contributions are:
\begin{itemize}
    \item We propose ACAM, a concept-based explainability module that effectively composes inductive biases from CNNs and ViTs to perform better model representation-concept alignment. 
    \item We demonstrate through quantitative experiments that ACAM improves both prediction accuracy and reduces concept-learning errors as compared to model-agnostic attention-based concept explainability modules across 7 different vision-transformer architectures.  
    \item We demonstrate through qualitative experiments that ACAM not only captures concept annotations missed by model-agnostic modules but also is robust to simple transformations and perturbations.
\end{itemize}



With the surge of advanced deep learning (DL) methods, deep neural networks (DNNs), especially Transformer-based networks \cite{vaswani2017attention}, have been widely deployed in human communities for the benefit of our life \cite{dargan2020survey,shorten2021deep}. In computer vision, Vision Transformers (ViT) show great scalability and impressive performance in various downstream tasks, which promotes its use in real-world applications like autonomous driving \cite{ando2023rangevit,dong2021image}. However, with the development and application of such advanced DNNs, there is a growing concern about their lack of interpretability and hesitation in applying the technology in high-stakes areas such as finance and healthcare. Given the current situation, a number of studies on the interpretability of DNNs have emerged \cite{li2022interpretable}.

% Posthoc vs Interpretable models

Current research on DNN interpretability can be broadly categorized into two classes. The first class is post-hoc interpretation, which includes model-agnostic methods that can be applied to trained models. Specifically, some post-hoc methods assign relative importance scores to different features considered \cite{ribeiro2016should,sundararajan2017axiomatic}, while some other approaches will rank the input training samples according to their importance to prediction \cite{koh2017understanding,ghorbani2019data}. Another class of methods tries to design intrinsically interpretable models. For example, various approaches have attempted to incorporate human-understandable concerts into model architecture and training processes. Concepts can be considered as shared abstract entities across multiple instances, which provide a general understanding of the task processed by the model. Many studies have explored how to integrate the model's decision-making process with task-relevant concepts to achieve transparent, interpretable model predictions \cite{koh2020concept,pedapati2020learning,jeyakumar2020can,heskes2020causal,o2020generative,kim2018interpretability,li2018deep,alvarez2018towards,chen2019looks}.

Concept-based explainability builds upon two distinct assumptions - (i) concepts are independent entities that are shared among multiple samples from the same class, and (ii) task performance can be directly computed using concept representations. In other words, given a set of concept representations $C$ associated with an input sample $x$, the task prediction is dependent on $y = g(C)$ where $g$ is any interpretable function used to aggregate concepts. Multiple works such as \cite{alvarez2018towards} and \cite{agarwal2021neural} have postulated using a weighted linear sum of concepts as $g$. Other works such as \cite{koh2020concept} have postulated using a shallow feed-forward network as mapping from concepts to prediction. 

% Advent of attention
With the success of attention mechanism \cite{vaswani2017attention} in designing large-scale networks for language\cite{devlin2018bert} and vision applications \cite{dosovitskiy2020image}, multiple diverse use-cases for attention have been proposed. Attention weights have been analyzed as an ``explanation'' for a particular data sample for large models \cite{mullenbach2018explainable}. While significant debate still looms over the veracity of using attention weights to explain ``features'' (tokens) \cite{jain2019attention, wiegreffe2019attention}, there is consensus among researchers that attention mechanism can reliably assign trustworthy relevance scores over a sequence of independent features. 

A particular use case of attention in concept-based explainability is utilizing the attention mechanism in modeling the concept aggregation function $g$ as first proposed in \cite{rigotti2021attention}. Note that concepts are independent entities shared among different training samples, hence attention can be reliably used to assign ``relevance'' scores to the concepts relative to a prediction. The Concept Transformer (CT) proposed by  \cite{rigotti2021attention} achieves better performance and provides better explanations than present SOTA methods. It is designed to be a classifier head and be agnostic to the features it receives from the backbone network. 
% Even though CT achieves SOTA performance on feature extraction backbones ranging from CNNs to Vision transformers (ViTs), it does not make any assumptions about the input features. This is a problem, because the features computed by a CNN are fundamentally different from features computed by a ViT.
Though CT achieves SOTA performance, the use of standard Vision Transformers (ViTs) \cite{dosovitskiy2020image} in this approach limits its awareness of the spatial information in images, hindering its modeling of concepts across different parts in the input.

In computer vision, ViTs \cite{dosovitskiy2020image} have been proposed as an alternative to traditional CNNs for large-scale vision applications. ViTs borrow their architecture from transformer-based language approaches \cite{vaswani2017attention,devlin2018bert}. A ViT first segments an image into equal patches, which are then projected into an embedding space. Subsequently, a pre-computed positional embedding is added to the patches which to encode information about their relative positions which are then concatenated into a sequence. The sequence is passed through stacked transformer blocks to compute a patch feature which is used in downstream tasks. ViTs have demonstrated better performance than CNNs, especially when pre-trained with large-scale data. However, due to the very architecture of ViTs being borrowed from language paradigm, they lack vision-specific \textit{inductive biases}. CNNs, which have been specifically designed for image modalities capture explicit inductive biases such as - scale invariance and transformation equivariance. Multiple approaches have been proposed to incorporate vision-specific inductive biases in ViTs like SWIN \cite{liu2021swin} and DETR \cite{zhu2020deformable}. However, all these approaches make significant changes in the model architecture.
% add some stuff about how vit>swin

In this paper, we propose a novel Spatially-aware Concept Transformer (SACT) module for providing concept-based explanations for ViTs. The SACT module effectively composes representations from a standard ViT with spatially-aware and scale-invariant representations from a CNN pipeline. In effect, SACT successfully combines inductive biases from both ViTs and CNNs - inter-patch relationships from ViT and spatial invariance and transform equivariance from CNNs. Our SACT module acts as a network-agnostic classification module on top of standard ViT architectures which improves prediction performance and explainability. The SACT consists of three distinct modules - the SPatial Awareness (SPA) module which extracts multi-scale features, the Multi-Scale Feature Interaction (MSFI) module which composes features from the ViT and SPA modules together using Deformable Attention, and the ConcePt Awareness (CPA) module which encapsulates global and spatial Concept-Patch attention units to perform downstream task predictions. Specifically, our paper makes the following contributions:
\begin{itemize}
    \item Our proposed work is the first to effectively combine inductive biases from both CNNs and ViTs in a standalone concept-based explainability module using an attention mechanism
    \item Our approach outperforms present state-of-the-art concept-based explanation approaches across three diverse datasets.
    \item Our approach provides more accurate explanations as compared to the previous approaches as compared to human-annotated concepts.
\end{itemize}

==> content/introduction_eccv.tex <==
\section{Introduction}
\label{sec:intro}

% Need for explainability

With the surge of advanced deep learning (DL) methods, deep neural networks (DNNs), especially Transformer-based networks \cite{vaswani2017attention}, have been widely deployed in human communities for the benefit of our life \cite{dargan2020survey,shorten2021deep}. In computer vision, Vision Transformers (ViT) show great scalability and impressive performance in various downstream tasks, which promotes its use in real-world applications like autonomous driving \cite{ando2023rangevit,dong2021image}. However, with the development and application of such advanced DNNs, there is a growing concern about their lack of interpretability and hesitation in applying the technology in high-stakes areas such as finance and healthcare. Given the current situation, a number of studies on the interpretability of DNNs have emerged \cite{li2022interpretable}.

% Posthoc vs Interpretable models

Current research on DNN interpretability can be broadly categorized into two classes. The first class is post-hoc interpretation, which includes model-agnostic methods that can be applied to trained models. Specifically, some post-hoc methods assign relative importance scores to different features considered \cite{ribeiro2016should,sundararajan2017axiomatic}, while some other approaches will rank the input training samples according to their importance to prediction \cite{koh2017understanding,ghorbani2019data}. Another class of methods tries to design intrinsically interpretable models. For example, various approaches have attempted to incorporate human-understandable concerts into model architecture and training processes. Concepts can be considered as shared abstract entities across multiple instances, which provide a general understanding of the task processed by the model. Many studies have explored how to integrate the model's decision-making process with task-relevant concepts to achieve transparent, interpretable model predictions \cite{koh2020concept,pedapati2020learning,jeyakumar2020can,heskes2020causal,o2020generative,kim2018interpretability,li2018deep,alvarez2018towards,chen2019looks}.

Concept-based explainability builds upon two distinct assumptions - (i) concepts are independent entities that are shared among multiple samples from the same class, and (ii) task performance can be directly computed using concept representations. In other words, given a set of concept representations $C$ associated with an input sample $x$, the task prediction is dependent on $y = g(C)$ where $g$ is any interpretable function used to aggregate concepts. Multiple works such as \cite{alvarez2018towards} and \cite{agarwal2021neural} have postulated using a weighted linear sum of concepts as $g$. Other works such as \cite{koh2020concept} have postulated using a shallow feed-forward network as mapping from concepts to prediction. 

% Advent of attention
With the success of attention mechanism \cite{vaswani2017attention} in designing large-scale networks for language \cite{devlin2018bert} and vision applications \cite{dosovitskiy2020image}, multiple diverse use-cases for attention have been proposed. Attention weights have been analyzed as an ``explanation'' for a particular data sample for large models \cite{mullenbach2018explainable}. While significant debate still looms over the veracity of using attention weights to explain ``features'' (tokens) \cite{jain2019attention, wiegreffe2019attention}, there is consensus among researchers that attention mechanism can reliably assign trustworthy relevance scores over a sequence of independent features. 

A particular use case of attention in concept-based explainability is utilizing the attention mechanism in modeling the concept aggregation function $g$ as first proposed in \cite{rigotti2021attention}. Note that concepts are independent entities shared among different training samples, hence attention can be reliably used to assign ``relevance'' scores to the concepts relative to a prediction. The Concept Transformer (CT) proposed by  \cite{rigotti2021attention} achieves better performance and provides better explanations than present SOTA methods. It is designed to be a classifier head and be agnostic to the features it receives from the backbone network. 
% Even though CT achieves SOTA performance on feature extraction backbones ranging from CNNs to Vision transformers (ViTs), it does not make any assumptions about the input features. This is a problem, because the features computed by a CNN are fundamentally different from features computed by a ViT.
Though CT achieves SOTA performance, the use of standard Vision Transformers (ViTs) \cite{dosovitskiy2020image} in this approach limits its awareness of the spatial information in images, hindering its modeling of concepts across different parts in the input.

In computer vision, ViTs \cite{dosovitskiy2020image} have been proposed as an alternative to traditional CNNs for large-scale vision applications. ViTs borrow their architecture from transformer-based language approaches \cite{vaswani2017attention,devlin2018bert}. A ViT first segments an image into equal patches, which are then projected into an embedding space. Subsequently, a pre-computed positional embedding is added to the patches which to encode information about their relative positions which are then concatenated into a sequence. The sequence is passed through stacked transformer blocks to compute a patch feature which is used in downstream tasks. ViTs have demonstrated better performance than CNNs, especially when pre-trained with large-scale data. However, due to the very architecture of ViTs being borrowed from language paradigm, they lack vision-specific \textit{inductive biases}. CNNs, which have been specifically designed for image modalities capture explicit inductive biases such as - scale invariance and transformation equivariance. Multiple approaches have been proposed to incorporate vision-specific inductive biases in ViTs like SWIN \cite{liu2021swin} and DETR \cite{zhu2020deformable}. However, all these approaches make significant changes in the model architecture.
% add some stuff about how vit>swin

In this paper, we propose a novel Spatially-aware Concept Transformer (SACT) module for providing concept-based explanations for ViTs. The SACT module effectively composes representations from a standard ViT with spatially-aware and scale-invariant representations from a CNN pipeline. In effect, SACT successfully combines inductive biases from both ViTs and CNNs - inter-patch relationships from ViT and spatial invariance and transform equivariance from CNNs. Our SACT module acts as a network-agnostic classification module on top of standard ViT architectures which improves prediction performance and explainability. The SACT consists of three distinct modules - the SPatial Awareness (SPA) module which extracts multi-scale features, the Multi-Scale Feature Interaction (MSFI) module which composes features from the ViT and SPA modules together using Deformable Attention, and the ConcePt Awareness (CPA) module which encapsulates global and spatial Concept-Patch attention units to perform downstream task predictions. Specifically, our paper makes the following contributions:

